Insider Knowledge: How Much Can RAG Systems Gain from Evaluation Secrets?

RAG systems are increasingly evaluated and optimized using LLM judges, an approach that is rapidly becoming the dominant paradigm for system assessment. Nugget-based approaches in particular are now embedded not only in evaluation frameworks but also in the architectures of RAG systems themselves. While this integration can lead to genuine improvements, it also creates a risk of faulty measurements due to circularity. In this paper, we investigate this risk through comparative experiments with nugget-based RAG systems, including Ginger and Crucible, against strong baselines such as GPT-Researcher. By deliberately modifying Crucible to generate outputs optimized for an LLM judge, we show that near-perfect evaluation scores can be achieved when elements of the evaluation - such as prompt templates or gold nuggets - are leaked or can be predicted. Our results highlight the importance of blind evaluation settings and methodological diversity to guard against mistaking metric overfitting for genuine system progress.

==> includes/rag-original-at60.tex <==
% % In preamble once:
% % \usepackage{pgfplots}
% % \pgfplotsset{compat=1.18}

% \begin{tikzpicture}
% \begin{axis}[
%   width=10cm, height=7cm,
%   font=\small,
%   xlabel={Umbrela Evaluation NDCG},
%   ylabel={Manual Evaluation NDCG},
%   xmin=0.55, xmax=0.85,
%   ymin=0.45, ymax=0.75,
%   xtick={0.55,0.60,0.65,0.70,0.75,0.80,0.85},
%   ytick={0.45,0.50,0.55,0.60,0.65,0.70,0.75},
%   tick label style={/pgf/number format/fixed},
%   grid=both,
%   grid style={line width=.2pt, draw=gray!25},
%   major grid style={line width=.2pt, draw=gray!35},
%   legend style={draw=none, fill=none, font=\small, at={(0.97,0.03)}, anchor=south east},
%   title={Original System (tau@60: 0.84)},
%   title style={yshift=4pt}
% ]

% % Non-LLM systems (neutral color)
% \addplot[
%   only marks,
%   mark=*,
%   mark size=1.6pt,
%   black!70
% ]
% table[
%   x=x_llm_ndcg,
%   y=y_human_ndcg,
%   col sep=comma,
%   % include only rows where is_llm == 0
%   row predicate/.code={\pgfplotstablegetelem{\coordindex}{is_llm}\of\tablestring%
%     \edef\flag{\pgfplotsretval}%
%     \ifnum\flag=0\relax\else\def\pgfplotstablerow{skip}\fi}
% ]{rag-original-at60.csv};

% % LLM-judge systems (red)
% \addplot[
%   only marks,
%   mark=*,
%   mark size=1.6pt,
%   red!80!black
% ]
% table[
%   x=x_llm_ndcg,
%   y=y_human_ndcg,
%   col sep=comma,
%   row predicate/.code={\pgfplotstablegetelem{\coordindex}{is_llm}\of\tablestring%
%     \edef\flag{\pgfplotsretval}%
%     \ifnum\flag=1\relax\else\def\pgfplotstablerow{skip}\fi}
% ]{rag-original-at60.csv};

% \legend{Non-LLM systems, LLM-judge systems}

% \end{axis}
% \end{tikzpicture}

% Preamble (once in your doc):
% \usepackage{pgfplots}
% \pgfplotsset{compat=1.18}
% \usepackage{booktabs}

% ---------- Inline data table (shared by both plots) ----------

\begin{small}

\pgfplotstableread[col sep=comma]{
name,x_orig,x_adul,y_orig,y_adul,is_llm
webis-01,0.801,0.9824,0.707,0.7255,0
fs4+monot5_listgalore.rag24.test_top100,0.8268,0.966,0.704,0.7236,0
fs4+monot5_rz.rag24.test_top100,0.7876,0.966,0.7038,0.7297,0
uwc2,0.8163,0.966,0.7018,0.7222,1
fs4+monot5_rg4o.rag24.test_top100,0.8476,0.966,0.6916,0.7247,0
monster,0.8161,0.9639,0.6888,0.7114,1
fs4+monot5_rl31-70b.rag24.test_top100,0.8007,0.966,0.6867,0.7168,0
webis-03,0.7766,0.9193,0.6793,0.7009,0
fs4_bm25+rocchio_snowael_snowaem_gtel+monot5_rrf+rz_rrf.rag24.test,0.7756,0.966,0.6787,0.7211,0
zeph_test_rag24_doc_query_expansion+rrf_Rtask,0.7432,0.8968,0.6736,0.6961,0
fs4+monot5.rag24.test_top100,0.7542,0.966,0.6639,0.7163,0
ielab-blender-llama70b-external-only,0.7673,0.9297,0.6631,0.7095,0
zeph_test_rag_rrf_expand_Rtask,0.7404,0.8986,0.6616,0.696,0
webis-04,0.7651,0.8913,0.6561,0.6689,0
webis-05,0.7776,0.9825,0.6541,0.6978,0
uwcCQAR,0.7619,0.9183,0.6508,0.6758,0
grill_fine_grained_rel_2_summaries_cohere,0.7429,0.9296,0.6467,0.6947,0
grill_fine_grained_rel_2_full_doc_cohere,0.7364,0.9246,0.6457,0.692,0
zeph_test_rag_rrf_raw_query_Rtrack,0.7361,0.8951,0.6437,0.6739,0
ielab-blender-llama70b,0.7281,0.9306,0.6435,0.7048,0
ldilab_repllama_listt5_pass3,0.7351,0.9111,0.6425,0.688,0
ldilab_repllama_listt5_pass4,0.7345,0.9111,0.6406,0.6873,0
ldilab_repllama_listt5_pass1,0.7339,0.9111,0.6404,0.6861,0
ldilab_repllama_listt5_pass2,0.7346,0.9111,0.6399,0.686,0
ielab-blender-llama70b-internal-only,0.7268,0.9237,0.6366,0.7018,0
grill_fine_grained_rel_2_summaries_rrf_bm25_cohere,0.7387,0.9318,0.6329,0.6955,0
uwcCQA,0.7392,0.9183,0.6312,0.6702,1
uwc1,0.8081,0.9289,0.6309,0.6726,1 
ASCITI_co_co,0.7108,0.9025,0.63,0.688,0
sim_and_rerank_v1,0.7108,0.9025,0.63,0.688,0
ielab-blender-llama8b,0.7171,0.9306,0.6283,0.7041,0
sim_and_rerank_200_docs,0.7101,0.9271,0.6279,0.7106,0
neurerank,0.7096,0.8892,0.6223,0.6795,0
UDInfolab.bge.query,0.709,0.9293,0.6214,0.6899,0
ielab-blender-llama70b-filtered,0.7505,0.9306,0.6202,0.6931,0
grill_fine_grained_rel_2_full_doc,0.706,0.8422,0.6202,0.6694,0
UDInfolab.bge.ranker,0.6917,0.907,0.6176,0.6832,0
grill_fine_grained_summaries,0.7073,0.8446,0.6108,0.6655,0
ielab-blender-llama8b-filtered,0.7077,0.9306,0.6074,0.6837,0
uwc0,0.7093,0.9255,0.6067,0.681,0
test.rag24.rrf.raw.query.MiniLM+BM25,0.6861,0.9577,0.6062,0.6827,0
test.rag24.rrf.expanded.BM25.MiniLM,0.6887,0.9588,0.6061,0.6864,0
ASCITI_co_bge,0.6858,0.9025,0.606,0.6885,0
ielab-bm25-stella-hybrid,0.6835,0.9083,0.6059,0.6933,0
uwcCQR,0.7193,0.9025,0.6039,0.6691,0
ASCITI_co_gpt,0.6967,0.9017,0.6004,0.6739,0
test.rag24.no.rrf.no.expansion,0.6811,0.9307,0.5993,0.6751,0
UDInfolab.bge.AnsAi,0.6991,0.9136,0.5868,0.6565,0
neu,0.6568,0.8892,0.5852,0.6687,0
uwcCQ,0.6776,0.9025,0.5823,0.6655,0
LAS-splade-mxbai,0.6838,0.8938,0.5813,0.6654,0
LAS_ENN_T5_RERANKED_MXBAI,0.6351,0.8324,0.5592,0.6259,0
ISIR-IRIT-GEN,0.63,0.7953,0.5381,0.6158,0
SPLADE+Gemini,0.68,0.8799,0.5352,0.6148,0
UDInfolab.bge,0.6001,0.8877,0.5315,0.6612,0
LAS_enn_t5,0.5824,0.8324,0.4855,0.618,0
SpladeV3_only,0.6028,0.8956,0.4845,0.6282,0
LAS-splade-mxbai-rrf,0.6092,0.8741,0.4819,0.6153,0
LAS_ann_t5_qdrant,0.5819,0.8319,0.4811,0.6143,0
SPLADE+Jina,0.4356,0.8956,0.3641,0.6184,0
SPLADE+BGEv2m3,0.4429,0.8956,0.3238,0.6083,0
}\allragdata

% ---------- PLOT 1: Original (x = \llmJudge{} original, y = Manual original) ----------
\begin{tikzpicture}
\begin{axis}[
  width=5.5cm, height=5cm,
  font=\tiny,
  xlabel={\llmJudge{} (NDCG)},
  ylabel={Human Evaluation (NDCG)},
  xmin=0.42, xmax=0.86,
  ymin=0.30, %xmaxy=0.74, % (typo-proofing: we'll set y explicitly next)
  ymin=0.30, ymax=0.74,
  xtick={0.45,0.55,0.65,0.75,0.85},
  ytick={0.35,0.45,0.55,0.65,0.75},
  tick label style={/pgf/number format/fixed},
  grid=both,
  grid style={line width=.2pt, draw=gray!25},
  major grid style={line width=.2pt, draw=gray!35},
  % legend style={draw=none, fill=none, font=\small, at={(0,1)}, anchor=north west},
  legend style={draw=none, fill=none, font=\small, at={(0,1)}, anchor=north west, align=left, legend cell align=left},
  title={Original Systems},
  title style={yshift=4pt}
]


% Other systems (neutral)
\addplot[
  only marks, mark=*, mark size=1pt, black!70
] table[
  x=x_orig, y=y_orig
] {\allragdata}
% filter out the LLM points by plotting them over in red:
;

% LLM-judge systems (red overlay)
\addplot[
  only marks, mark=*, mark size=1pt, blue!30!cyan
] table[
  x=x_orig, y=y_orig
] {%
name x_orig y_orig
uwc2 0.8163 0.7018
monster 0.8161 0.6888
uwcCQA 0.7392 0.6312
uwc1 0.8081 0.6309
};
\legend{\tiny{Systems}, \tiny{... with} \tiny{\llmJudge{}}}

\end{axis}
\end{tikzpicture}
\end{small}

==> includes/rag-reranked-at60.tex <==
% \begin{tikzpicture}
% \begin{axis}[
%   width=10cm, height=7cm,
%   font=\small,
%   xlabel={Umbrela Evaluation NDCG},
%   ylabel={Manual Evaluation NDCG},
%   xmin=0.70, xmax=1.00,
%   ymin=0.60, ymax=0.75,
%   xtick={0.70,0.75,0.80,0.85,0.90,0.95,1.00},
%   ytick={0.60,0.65,0.70,0.75},
%   tick label style={/pgf/number format/fixed},
%   grid=both,
%   grid style={line width=.2pt, draw=gray!25},
%   major grid style={line width=.2pt, draw=gray!35},
%   legend style={draw=none, fill=none, font=\small, at={(0.97,0.03)}, anchor=south east},
%   title={Re-ranked with Umbrela (tau@60: 0.63)},
%   title style={yshift=4pt}
% ]

% % Non-LLM systems (neutral)
% \addplot[
%   only marks,
%   mark=*,
%   mark size=1.6pt,
%   black!70
% ]
% table[
%   x=x_llm_ndcg,
%   y=y_human_ndcg,
%   col sep=comma,
%   row predicate/.code={\pgfplotstablegetelem{\coordindex}{is_llm}\of\tablestring%
%     \edef\flag{\pgfplotsretval}%
%     \ifnum\flag=0\relax\else\def\pgfplotstablerow{skip}\fi}
% ]{rag-reranked-at60.csv};

% % LLM-judge systems (red)
% \addplot[
%   only marks,
%   mark=*,
%   mark size=1.6pt,
%   red!80!black
% ]
% table[
%   x=x_llm_ndcg,
%   y=y_human_ndcg,
%   col sep=comma,
%   row predicate/.code={\pgfplotstablegetelem{\coordindex}{is_llm}\of\tablestring%
%     \edef\flag{\pgfplotsretval}%
%     \ifnum\flag=1\relax\else\def\pgfplotstablerow{skip}\fi}
% ]{rag-reranked-at60.csv};

% \legend{Non-LLM systems, LLM-judge systems}

% \end{axis}
% \end{tikzpicture}

% ---------- Inline data table (shared by both plots) ----------
\pgfplotstableread[col sep=comma]{
name,x_orig,x_adul,y_orig,y_adul,is_llm
webis-01,0.801,0.9824,0.707,0.7255,0
fs4+monot5_listgalore.rag24.test_top100,0.8268,0.966,0.704,0.7236,0
fs4+monot5_rz.rag24.test_top100,0.7876,0.966,0.7038,0.7297,0
uwc2,0.8163,0.966,0.7018,0.7222,1
fs4+monot5_rg4o.rag24.test_top100,0.8476,0.966,0.6916,0.7247,0
monster,0.8161,0.9639,0.6888,0.7114,1
fs4+monot5_rl31-70b.rag24.test_top100,0.8007,0.966,0.6867,0.7168,0
webis-03,0.7766,0.9193,0.6793,0.7009,0
fs4_bm25+rocchio_snowael_snowaem_gtel+monot5_rrf+rz_rrf.rag24.test,0.7756,0.966,0.6787,0.7211,0
zeph_test_rag24_doc_query_expansion+rrf_Rtask,0.7432,0.8968,0.6736,0.6961,0
fs4+monot5.rag24.test_top100,0.7542,0.966,0.6639,0.7163,0
ielab-blender-llama70b-external-only,0.7673,0.9297,0.6631,0.7095,0
zeph_test_rag_rrf_expand_Rtask,0.7404,0.8986,0.6616,0.696,0
webis-04,0.7651,0.8913,0.6561,0.6689,0
webis-05,0.7776,0.9825,0.6541,0.6978,0
uwcCQAR,0.7619,0.9183,0.6508,0.6758,0
grill_fine_grained_rel_2_summaries_cohere,0.7429,0.9296,0.6467,0.6947,0
grill_fine_grained_rel_2_full_doc_cohere,0.7364,0.9246,0.6457,0.692,0
zeph_test_rag_rrf_raw_query_Rtrack,0.7361,0.8951,0.6437,0.6739,0
ielab-blender-llama70b,0.7281,0.9306,0.6435,0.7048,0
ldilab_repllama_listt5_pass3,0.7351,0.9111,0.6425,0.688,0
ldilab_repllama_listt5_pass4,0.7345,0.9111,0.6406,0.6873,0
ldilab_repllama_listt5_pass1,0.7339,0.9111,0.6404,0.6861,0
ldilab_repllama_listt5_pass2,0.7346,0.9111,0.6399,0.686,0
ielab-blender-llama70b-internal-only,0.7268,0.9237,0.6366,0.7018,0
grill_fine_grained_rel_2_summaries_rrf_bm25_cohere,0.7387,0.9318,0.6329,0.6955,0
uwcCQA,0.7392,0.9183,0.6312,0.6702,1
uwc1,0.8081,0.9289,0.6309,0.6726,1 
ASCITI_co_co,0.7108,0.9025,0.63,0.688,0
sim_and_rerank_v1,0.7108,0.9025,0.63,0.688,0
ielab-blender-llama8b,0.7171,0.9306,0.6283,0.7041,0
sim_and_rerank_200_docs,0.7101,0.9271,0.6279,0.7106,0
neurerank,0.7096,0.8892,0.6223,0.6795,0
UDInfolab.bge.query,0.709,0.9293,0.6214,0.6899,0
ielab-blender-llama70b-filtered,0.7505,0.9306,0.6202,0.6931,0
grill_fine_grained_rel_2_full_doc,0.706,0.8422,0.6202,0.6694,0
UDInfolab.bge.ranker,0.6917,0.907,0.6176,0.6832,0
grill_fine_grained_summaries,0.7073,0.8446,0.6108,0.6655,0
ielab-blender-llama8b-filtered,0.7077,0.9306,0.6074,0.6837,0
uwc0,0.7093,0.9255,0.6067,0.681,0
test.rag24.rrf.raw.query.MiniLM+BM25,0.6861,0.9577,0.6062,0.6827,0
test.rag24.rrf.expanded.BM25.MiniLM,0.6887,0.9588,0.6061,0.6864,0
ASCITI_co_bge,0.6858,0.9025,0.606,0.6885,0
ielab-bm25-stella-hybrid,0.6835,0.9083,0.6059,0.6933,0
uwcCQR,0.7193,0.9025,0.6039,0.6691,0
ASCITI_co_gpt,0.6967,0.9017,0.6004,0.6739,0
test.rag24.no.rrf.no.expansion,0.6811,0.9307,0.5993,0.6751,0
UDInfolab.bge.AnsAi,0.6991,0.9136,0.5868,0.6565,0
neu,0.6568,0.8892,0.5852,0.6687,0
uwcCQ,0.6776,0.9025,0.5823,0.6655,0
LAS-splade-mxbai,0.6838,0.8938,0.5813,0.6654,0
LAS_ENN_T5_RERANKED_MXBAI,0.6351,0.8324,0.5592,0.6259,0
ISIR-IRIT-GEN,0.63,0.7953,0.5381,0.6158,0
SPLADE+Gemini,0.68,0.8799,0.5352,0.6148,0
UDInfolab.bge,0.6001,0.8877,0.5315,0.6612,0
LAS_enn_t5,0.5824,0.8324,0.4855,0.618,0
SpladeV3_only,0.6028,0.8956,0.4845,0.6282,0
LAS-splade-mxbai-rrf,0.6092,0.8741,0.4819,0.6153,0
LAS_ann_t5_qdrant,0.5819,0.8319,0.4811,0.6143,0
SPLADE+Jina,0.4356,0.8956,0.3641,0.6184,0
SPLADE+BGEv2m3,0.4429,0.8956,0.3238,0.6083,0
}\allragdata

% ---------- PLOT 2: Adulterated (x = \llmJudge{} adulterated, y = Manual adulterated) ----------
\begin{tikzpicture}
\begin{axis}[
  % width=6cm, height=6cm,
  % font=\footnotesize,
   width=5.5cm, height=5cm,
  font=\tiny,
  xlabel={\llmJudge{} (NDCG)},
  ylabel={Human Evaluation (NDCG)},
  xmin=0.79, xmax=0.99,
  ymin=0.60, ymax=0.74,
  xtick={0.80,0.85,0.90,0.95,0.99},
  ytick={0.60,0.65,0.70,0.74},
  tick label style={/pgf/number format/fixed},
  grid=both,
  grid style={line width=.2pt, draw=gray!25},
  major grid style={line width=.2pt, draw=gray!35},
  legend style={draw=none, fill=none, font=\small, at={(0,1)}, anchor=north west, align=left, legend cell align=left}
  ,  title={Adulterated Systems},
  title style={yshift=4pt}
]

% Other systems (neutral)
\addplot[
  only marks, mark=*, mark size=1pt, black!70
] table[
  x=x_adul, y=y_adul
] {\allragdata};

% LLM-judge systems (red overlay)
\addplot[
  only marks, mark=*, mark size=1pt, blue!30!cyan
] table[
  x=x_adul, y=y_adul
] {%
name x_adul y_adul
uwc2 0.966 0.7222
monster 0.9639 0.7114
uwcCQA 0.9183 0.6702
uwc1 0.9289 0.6726
};

\legend{\tiny{Systems}, \tiny{... with} \tiny{\llmJudge{}}}

% \legend{Systems, Systems with \\ \llmJudge{}}
\end{axis}
\end{tikzpicture}

